Scientific Opinion Summarization: Paper Meta-review Generation Dataset, Methods, and Evaluation

Opinions in scientific research papers can be divergent, leading to controversies among reviewers. However, most existing datasets for opinion summarization are centered around product reviews and assume that the analyzed opinions are non-controversial, failing to account for the variability seen in other contexts such as academic papers, political debates, or social media discussions. To address this gap, we propose the task of scientific opinion summarization, where research paper reviews are synthesized into meta-reviews. To facilitate this task, we introduce the ORSUM dataset covering 15,062 paper meta-reviews and 57,536 paper reviews from 47 conferences. Furthermore, we propose the Checklist-guided Iterative Introspection approach, which breaks down scientific opinion summarization into several stages, iteratively refining the summary under the guidance of questions from a checklist. Our experiments show that (1) human-written summaries do not always satisfy all necessary criteria such as depth of discussion, and identifying consensus and controversy for the specific domain, and (2) the combination of task decomposition and iterative self-refinement shows strong potential for enhancing the opinions and can be applied to other complex text generation using black-box LLMs.

==> tables/dialogue_chatgpt_metareview.tex <==
\begin{table*}[htb]
\small
\centering
\begin{tabular}{lp{12cm}}
\toprule[1pt]
Step 1 & From the sentiments and aspects discussed in the reviews, what are the key strengths and weaknesses of this paper? Please cite corresponding reviewers and evidence) \\
\hline
 & Based on the reviews, the key strengths of the paper include the proposal of a technically simple yet comprehensive approach to neural process models that can produce correlated predictions, capture non-Gaussian output distributions, and support multiple outputs. The use of invertible transformations is also highlighted as a strength of the model. The experiments conducted on artificial and real data demonstrate the advantages of the proposed model over related models, such as the fullConvGNP model, and its ability to outperform mean field, convNP.\\
\hline
Step 2 & Identify the points of agreement and disagreement among the reviewers. Please include the corresponding reviewers and evidence.\\
\hline
 & Based on the reviews, the key strengths of the paper include addressing a core issue of conditional neural processes by proposing a model that captures dependencies between test points, using structured Gaussian covariances and a Gaussian copula model. The authors demonstrate through experiments that modeling these dependencies improves the performance of the model on various datasets. The approach is also seen as technically sound and well-motivated. However, the paper is criticized for not using a normalizing flow model.\\
\hline
Step 3 & Considering the key sentiments from the reviews, the identified strengths and weaknesses, and the consensus and controversy among the reviewers, write a metareview with decision of acceptance/rejection.\\
\hline
 & Based on the reviews, the key strengths of the paper include the ease of understanding and implementation of the proposed methods, the improvement in performance due to modeling dependencies through a covariance function, and the ability to handle non-Gaussian distributions using Copulae. The experiments conducted on multiple datasets demonstrate the effectiveness of modeling dependencies in the input and output. However, the paper is criticized for lacking novelty in the proposed methods, which are seen as a direct implementation of a Gaussian process with deep kernel learning.\\
\hline
Q1 & Are the most important advantages and disadvantages discussed in the above meta-review? Are the most important consensus and controversy discussed in the above meta-review? Is the above meta-review contradicting reviewers' comments? Is the above meta-review supporting the rejection decision? If not, how can it be improved? \\
\hline
 & Agreement: - The proposed methods are technically sound and easy to understand and implement. (Reviewer 1, 3) - The modeling of dependencies through a covariance function improves the performance of the model. (Reviewer 1, 2, 3) - The ability to handle non-Gaussian distributions using Copulae is a strength of the proposed methods. (Reviewer 1, 2, 3) - The experiments conducted on multiple datasets demonstrate the effectiveness of modeling dependencies. \\
\hline
step 4 & using this discussion, write an accurate <200 words metareview with decision of acceptance/rejection.\\
\hline
 & After carefully considering the sentiments from the reviews, the identified strengths and weaknesses, as well as the consensus and controversy among the reviewers, we have decided to accept the paper for publication with minor revisions. The proposed methods for modeling dependencies in the input and output through a covariance function are technically sound and easy to understand and implement. The ability to handle non-Gaussian distributions using Copulae is also a strength of the proposed methods. The experiments conducted on multiple datasets demonstrate the effectiveness of the proposed methods in improving the performance of the model.While some reviewers have raised concerns about the novelty of the proposed methods, the technical soundness and effectiveness of the proposed methods in modeling dependencies and handling non-Gaussian distributions are sufficient for acceptance.Minor revisions are required to address.\\
\hline
Q2 & Are the most important advantages and disadvantages discussed in the above meta-review? Are the most important consensus and controversy discussed in the above meta-review? Is the above meta-review contradicting reviewers' comments? Is the above meta-review supporting the rejection decision? If not, how can it be improved? \\
\hline
 & Yes, the most important advantages and disadvantages of the paper are discussed in the meta-review. The main strengths include the technical soundness of the proposed methods, the ability to handle non-Gaussian distributions using Copulae, and the improvement in performance due to the modeling of dependencies through a covariance function. The main weakness is the lack of novelty in the proposed methods. The meta-review discusses both consensus and controversy among the reviewers. There is a consensus about the technical soundness and effectiveness of the proposed methods in modeling dependencies and handling non-Gaussian distributions. However, there is controversy about the novelty of the proposed methods and the adequacy of the experiments and analyses. The meta-review does not contradict any reviewers' comments, but rather integrates and summarizes them. \\
\hline
Q3 & using this discussion, write an accurate <200 words metareview with the decision of acceptance/rejection.\\
\hline
 & The paper proposes variants of Neural process (NP) that can model correlation in the input and output for multi-output regression. The proposed methods involve directly parameterizing the mean and the covariance functions of a Gaussian predictive via neural networks and using Copulae to handle non-Gaussian marginal distributions. The paper presents comprehensive experiments on multiple datasets, demonstrating the effectiveness of the proposed methods in improving the performance of the model.While some reviewers have raised concerns about the novelty of the proposed methods, the technical soundness and effectiveness of the proposed methods in modeling dependencies and handling non-Gaussian distributions are sufficient for acceptance. The proposed methods are technically sound and easy to understand and implement, and the ability to handle non-Gaussian distributions using Copulae is a strength of the proposed methods. The modeling of dependencies through a covariance function improves the performance of the model, which is further demonstrated through comprehensive experiments on multiple datasets.Minor revisions are required to address some specific concerns raised by the reviewers. Therefore, we recommend acceptance of the paper.\\
\hline
 & After a thorough review of the paper and the opinions of the reviewers, we have decided to accept the manuscript for publication with minor revisions.The proposed methods for modeling dependencies in the input and output through a covariance function are technically sound and easy to understand and implement. The ability to handle non-Gaussian distributions using Copulae is also a strength of the proposed methods. The experiments conducted on multiple datasets demonstrate the effectiveness of the proposed methods in improving the performance of the model.While some reviewers have raised concerns about the novelty of the proposed methods, the technical soundness and effectiveness of the proposed methods in modeling dependencies and handling non-Gaussian distributions are sufficient for acceptance. The minor revisions required include clarifying the differences between the proposed methods and related work and providing more quantitative analysis of the results.Overall, we believe that the proposed methods have the potential to advance the field of neural processes and will be of interest to the community.\\
\hline
\bottomrule[1pt]
\end{tabular}
\caption{
Prompts for all Prompting Models
}
\label{table:Prompt}
\end{table*}

==> tables/prompts.tex <==
\begin{table*}[htb]
\small
\centering
\begin{tabular}{lp{12cm}}
\toprule[1pt]
\textbf{Models} & \textbf{Prompts} \\
\hline
Vanilla & Generate a Metareview\\
\hline
3sent & Generate a summary of document in 3 sentences.\\
\hline
InstructPrompt & Imagine you are a human metareviewer now. You will write metareviews for a conference. Please follow these steps:
1. Carefully read the reviews, and be aware of the information it contains.
2. Generate a metareview based on three dimensions: 'Discussion Involvement', 'Opinion Faithfulness' and 'Decision Consistency'. 
Definitions are as follows:
(1) Discussion Involvement: Discuss the paper's strengths and weaknesses, as well as agreements and disagreements among reviewers,
(2) Opinion Faithfulness: Do not contradict reviewers' comments,
(3) Decision Consistency: Accurately reflect the final decisions.\\
\hline
TCG & Describe	the	topic	of	each	sentence in	one	word. Summarize	what	reviewers	said of	the	paper. Summarize the summaries of the reviews\\
\hline
ICL & Given a pair of reviews and a metareview as an example, Generate a metareview based on given reviews. \{example\}\\
\hline
\textbf{CGI$^2$} (ours) & From the sentiments and aspects discussed in the reviews, what are the key strengths and weaknesses of this paper? Please cite corresponding reviewers and evidence. Identify the points of agreement and disagreement among the reviewers. Please include the corresponding reviewers and evidence. Considering the key sentiments from the reviews, the identified strengths and weaknesses, and the consensus and controversy among the reviewers, write a metareview with decision of acceptance/rejection. Are the most important advantages and disadvantages discussed in the above meta-review? Are the most important consensus and controversy discussed in the above meta-review? Is the above meta-review contradicting reviewers' comments? Is the above meta-review supporting the rejection decision? If not, how can it be improved? using this discussion, write an accurate <200 words metareview with decision of acceptance/rejection.
 \\
 \hline
CGI$^2$ ablation & From the sentiments and aspects discussed in the reviews, what are the key strengths and weaknesses of this paper? Please cite corresponding reviewers and evidence. Identify the points of agreement and disagreement among the reviewers. Please include the corresponding reviewers and evidence. Considering the key sentiments from the reviews, the identified strengths and weaknesses, and the consensus and controversy among the reviewers, write a metareview with decision of acceptance/rejection.\\
\bottomrule[1pt]
\end{tabular}
\caption{
Prompts we use in all prompting-based methods.
}
\label{table:prompts}
\end{table*}
